MLPnP - A Real-Time Maximum Likelihood Solution to the Perspective-n-Point Problem

In this paper, a statistically optimal solution to the Perspective-n-Point (PnP) problem is presented. Many solutions to the PnP problem are geometrically optimal, but do not consider the uncertainties of the observations. In addition, it would be desirable to have an internal estimation of the accuracy of the estimated rotation and translation parameters of the camera pose. Thus, we propose a novel maximum likelihood solution to the PnP problem, that incorporates image observation uncertainties and remains real-time capable at the same time. Further, the presented method is general, as is works with 3D direction vectors instead of 2D image points and is thus able to cope with arbitrary central camera models. This is achieved by projecting (and thus reducing) the covariance matrices of the observations to the corresponding vector tangent space.

==> NullSpaceMethod.tex <==
Let a world point $mathbf{p}_i \in \mathbb{R}^3$ be observed by a calibrated camera and let the uncertain observation be 
\begin{equation}
\mathbf{x} =
\begin{bmatrix}	
x\\y\\1
\end{bmatrix}
,
\mathbf{\Sigma}_{xx} =
\begin{bmatrix}	
\sigma^2_x , \sigma_xy\\\sigma_yx \sigma^2_y
\end{bmatrix}
\end{equation}
with covariance $\mathbf{\Sigma}_{xx}$.
%Further, the euclidean transformation from the camera to the world frame is given by a rotation $\mathbf{R} \in SO(3)$ and a translation $\mathbf{t}$.
%The 
%
%Assuming a calibrated camera, a $\mathbf{x}=[x,y,1]^{T}$ with uncertainty $\mathbf{\Sigma}_{xx}$ on the  image plane. 
%
%Its corresponding bearing vector is g
%Given two images (left and right) with corresponding bearing vectors (camera rays):
%\begin{equation}
%\mathbf{X}_l =
%\begin{bmatrix}	
% 	 x_l\\ y_l\\ z_l
%\end{bmatrix} 
%\mathbf{X}_r =
%\begin{bmatrix}	
% 	x_r \\y_r\\z_r
%\end{bmatrix}
%\end{equation}
We are looking for is the mapping of $\mathbf{X}_l$ to $\mathbf{X}_r$: 
\begin{equation}
\mathbf{X}_r =
\mathbf{R} \cdot \mathbf{X}_l + \mathbf{T} =
\begin{bmatrix}	
 	 r_{11} r_{12} r_{13}\\
	 r_{21} r_{22} r_{23}\\
	 r_{31} r_{32} r_{33}\\
\end{bmatrix} 
\begin{bmatrix}	
 	x_l\\y_l\\z_l
\end{bmatrix} 
+
\begin{bmatrix}	
 	t_1\\t_2\\t_3
\end{bmatrix}
\end{equation}
where $\mathbf{R}$ is a $3\times3$ rotation and $T$ a $3\times1$ translation vector, i.e. 12 unknowns.
\par
\par
We write the calculation of a nullspace vectors as: 
\begin{equation}
\begin{bmatrix}	
 	\mathbf{\alpha}, \mathbf{\beta} 
\end{bmatrix}
= null(\mathbf{X}^T)
\end{equation}
where:
\begin{equation}
\mathbf{\alpha} = 
\begin{bmatrix}	
 	\alpha_1 \\ \alpha_2 \\ \alpha_3
\end{bmatrix}
\mathbf{\beta} = 
\begin{bmatrix}	
 	\beta_1 \\ \beta_2 \\ \beta_3
\end{bmatrix}
\end{equation}

Next we can calculate the tangent space of both vectors, i.e. the two nullspace vectors of both vectors:
\begin{equation}
\begin{bmatrix}	
 	\mathbf{\alpha}_l, \mathbf{\beta}_l
\end{bmatrix}
= null(\mathbf{X}_l^T)
\end{equation}
\begin{equation}
\begin{bmatrix}	
 	\mathbf{\alpha}_r, \mathbf{\beta}_r
\end{bmatrix}
= null(\mathbf{X}_r^T)
\end{equation}

The next step is the calculation of the tangent space residuals after projecting the bearing vector from the left to the right camera:
\begin{equation}
\begin{bmatrix}	
 	\mathbf{\alpha}_r, \mathbf{\beta}_r
\end{bmatrix}
= null(\mathbf{X}_r^T)
\end{equation}
The residuals of t





